Integrating Static Code Analysis Toolchains

This paper proposes an approach for a tool-agnostic and heterogeneous static code analysis toolchain in combination with an exchange format. This approach enhances both traceability and comparability of analysis results. State of the art toolchains support features for either test execution and build automation or traceability between tests, requirements and design information. Our approach combines all those features and extends traceability to the source code level, incorporating static code analysis. As part of our approach we introduce the "ASSUME Static Code Analysis tool exchange format" that facilitates the comparability of different static code analysis results. We demonstrate how this approach enhances the usability and efficiency of static code analysis in a development process. On the one hand, our approach enables the exchange of results and evaluations between static code analysis tools. On the other hand, it enables a complete traceability between requirements, designs, implementation, and the results of static code analysis. Within our approach we also propose an OSLC specification for static code analysis tools and an OSLC communication framework.

==> enduserperspective.tex <==
% !TEX root =  Main.tex
\section{The end-user perspective of our approach}
\label{sec:enduserPerspective}
This section presents our approach from an end-user perspective to show how complexity is hidden from the end-user. Figure \ref{fig:mockUp} shows a mock-up of a prospective user interface, which supports the developer to browse quickly through different modules and versions of the corresponding files and analysis results. In the rest of this section, a possible process without traceability is presented, with the two roles, developer and analysis expert, to bring out the advantages of our proposed process. After that, the workflow of the toolchain is explained considering the mock-up.

A possible process for developing and analyzing C-code without a toolchain could start after corresponding detail design activities (cf. Figure~\ref{fig:vModell}). During the implementation activity, the developers transfer the design specifications into C-code. After that, an analysis expert configures the analysis tool to match a specific type of processor and performs the \textit{static code analysis}. After the code is analyzed the analysis experts send the \textit{analysis report} to the developers via e-mail. In the next step the developers fix all detected problems. Afterwards, the analysis expert analyses the code again and e-mails the report back again. This step is repeated until no errors occur in the analysis report. Because there is only one report for each analysis and the developers are working on different files, they have to locate repeatedly the right checks referring to their files in the current report. Furthermore, the analysis expert has to ensure that the right versions of the files are analyzed. This process is error-prone and time-consuming.

To cope with these challenges a process with an analysis toolchain is proposed in the following.
A Developer writes code in an IDE and manages its versions with a version management system like Git. An analysis expert creates an \texttt{Analysis Case}. Within an \texttt{Analysis Case} the analysis configuration is defined and a collection of files that should be analyzed. For every version that the developer pushes into the repository, the toolchain produces \texttt{Analysis Results}. Therefore, the Analysis Client is triggered and check each \texttt{Analysis Case} whether it is effected by the changes in the repository or not. The Analysis Client triggers the analysis tool and pushes it into the corresponding repository. This triggers the Analysis Adapter that produces the \texttt{Analysis Result} and links it with the corresponding files. The developer can use a web application, similar to the mock-up in Figure~\ref{fig:mockUp}, to get a view of all \texttt{Analysis Cases}. For each \texttt{Analysis Case}, he gets a list of all available \texttt{Analysis Results} and for each \texttt{Analysis Result} he gets all files belonging to the \texttt{Analysis Case}. Furthermore, he sees a status flag on each file. A red flag means that the static analysis tool found an error and a green flag that no errors were detected. Additionally, he can have a closer look at each file via an integrated viewer (not shown in the mock-up). This viewer shows the content of a selected file with line numbers and flags on each line number. The flags shows whether there is an error at a specific location in the code or not. Via the red error-flags in this view, the developer can get more detail information about an error. In this way, the developer can quickly find all errors for different modules defined in an \texttt{Analysis Case} and solve the errors. After he pushed the corrected versions to the server, the analysis starts again, and after the analysis is done he can directly get the results of the analysis and prove if his bug fix has worked out. Additionally as shown in the mock-up, there could be used different analysis tools. The selection of an analysis tool could also be defined in an \texttt{Analysis Case}. In that way, the results of different analysis tools could be compared.

%TODO insert figure with Mock-Up
\begin{figure}[ht]
\centering
\vspace*{-1.0em}
\includegraphics[width=\linewidth]{Figures/MockUp.png}
\vspace*{-1.0em}
\caption{Mock-Up web based application for usability}\label{fig:mockUp}
\vspace*{-1.3em}
\end{figure}



==> implementation.tex <==
% !TEX root =  Main.tex
\section{Implementation} 
\label{sec:impl}
The platform has been implemented in ...

==> motivatingexample.tex <==
\section{Motivating Example} \label{motivation}


